Cosmological correlators from the Euclidean sphere

We propose a new framework for computing late-time cosmological correlators in de Sitter spacetime by analytic continuation from the Euclidean sphere. In this framework, correlators of arbitrary massive scalar fields take the universal form of generalized Euler integrals. Using this representation, we reproduce the results obtained using the Schwinger-Keldysh formalism for a range of tree-level and loop diagrams, providing nontrivial checks of the equivalence between the Euclidean and the in-in formalisms. We further show that a Landau analysis of the generalized Euler integrals determines the singularities of the corresponding correlators in momentum space. This framework provides a systematic approach to studying the analytic structure of cosmological correlators.

==> affiliation_icons.tex <==
\RequirePackage{tikz}

\protected\def\SphereIcon{
  \begin{tikzpicture}[
    x=.85em,y=.85em,
    baseline=(current bounding box.south),
    line cap=round,line join=round,
    draw=black,line width=.035em]
    \path[use as bounding box] (-.56,-.56) rectangle (.56,.56);
    \draw (0,0) circle[radius=.5];
    \draw[line width=.022em,dash pattern=on .05em off .04em]
      (.5,0) arc[start angle=0,end angle=180,x radius=.5,y radius=.16];
    \draw[line width=.026em]
      (-.5,0) arc[start angle=180,end angle=360,x radius=.5,y radius=.16];
  \end{tikzpicture}
}

\protected\def\dSIcon{
  \begin{tikzpicture}[
    x=.85em,y=.85em,
    baseline=(current bounding box.south),
    line cap=round,line join=round,
    draw=black,line width=.035em]
    \path[use as bounding box] (-.56,-.56) rectangle (.56,.56);
    \draw plot[domain=-.45:.45,samples=25,variable=\t]
      ({sqrt(.0484+\t*\t)},\t);
    \draw plot[domain=-.45:.45,samples=25,variable=\t]
      ({-sqrt(.0484+\t*\t)},\t);
    \draw[line width=.026em]
      (0,.45) ellipse[x radius=.5009,y radius=.105];
    \draw[line width=.022em,dash pattern=on .05em off .04em]
      (.5009,-.45)
      arc[start angle=0,end angle=180,x radius=.5009,y radius=.105];
    \draw[line width=.026em]
      (-.5009,-.45)
      arc[start angle=180,end angle=360,x radius=.5009,y radius=.105];
    \draw[line width=.022em,dash pattern=on .05em off .04em]
      (.22,0) arc[start angle=0,end angle=180,x radius=.22,y radius=.06];
    \draw[line width=.026em]
      (-.22,0) arc[start angle=180,end angle=360,x radius=.22,y radius=.06];
  \end{tikzpicture}
}


\protected\def\SphereAffil{\textsuperscript{\SphereIcon}}
\protected\def\dSAffil{\textsuperscript{\dSIcon}}


\AddToHook{package/hyperref/after}{
  \pdfstringdefDisableCommands{
    \def\SphereIcon{S}
    \def\dSIcon{dS}
    \def\SphereAffil{}
    \def\dSAffil{}
  }
}

\protected\long\def\AffiliationRow#1#2{
  \leavevmode
  \hbox{
    \makebox[1.6em][l]{#1}
    \parbox[t]{.90\textwidth}{\raggedright #2\par}
  }
}

\AddToHook{package/hyperref/after}{
  \pdfstringdefDisableCommands{
    \def\AffiliationRow#1#2{#2}
  }
}
